Security for the Industrial IoT: The Case for Information-Centric Networking

Industrial production plants traditionally include sensors for monitoring or documenting processes, and actuators for enabling corrective actions in cases of misconfigurations, failures, or dangerous events. With the advent of the IoT, embedded controllers link these `things' to local networks that often are of low power wireless kind, and are interconnected via gateways to some cloud from the global Internet. Inter-networked sensors and actuators in the industrial IoT form a critical subsystem while frequently operating under harsh conditions. It is currently under debate how to approach inter-networking of critical industrial components in a safe and secure manner. In this paper, we analyze the potentials of ICN for providing a secure and robust networking solution for constrained controllers in industrial safety systems. We showcase hazardous gas sensing in widespread industrial environments, such as refineries, and compare with IP-based approaches such as CoAP and MQTT. Our findings indicate that the content-centric security model, as well as enhanced DoS resistance are important arguments for deploying Information Centric Networking in a safety-critical industrial IoT. Evaluation of the crypto efforts on the RIOT operating system for content security reveal its feasibility for common deployment scenarios.

==> figures/initial.tex <==
\begin{tikzpicture}[tpic]
    \pic {topo=t/hide/node/0};
    \path[->] (t-E) edge (t-C) (t-C) edge (t-D) (t-D) edge (t-B) (t-B) edge (t-R);
    \path[-,dashed] (t-R) edge (t-CL) (t-CL.-135) edge (t-DV);
\end{tikzpicture}


==> figures/styles.tex <==
\def\DIST{5em}
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}
\tikzset{
    tpic/.style = {font=\sffamily,>={Latex}},
    node/.style = {circle,minimum width=2em,draw,fill=purple!30,inner sep=1pt},
    inactive/.style = {node,draw=black,fill=black!10,dashed},
    hide/.style = {text opacity=0},
    root/.style = {node,double,fill=red!30},
    cl/.style = {font=\sffamily\huge,cloud,cloud puffs=15.7,cloud ignores aspect,draw,fill=gray!20,inner sep=2pt},
    labels/.style = {sloped,font=\sffamily,pos=0.68,inner xsep=0pt,text=black!40},
    mqttBG/.style = {fill=black!5,labels},
    tablet/.pic = {
        \draw[line width=1pt,rounded corners=3pt] (0,0) rectangle (0.75,1);
        \draw[line width=1pt] (0.1,0.2) rectangle (0.65,0.9);
        \fill (0.375,0.1) circle (1pt);
        \fill (0.375,0.4) circle (1pt);
        \draw[line width=1pt]
            ([shift=(45:0.1)]0.375,0.4) arc (45:135:0.1)
            ([shift=(45:0.175)]0.375,0.4) arc (45:135:0.175)
            ([shift=(45:0.25)]0.375,0.4) arc (45:135:0.25);
            \node[fit={(0,0)(0.75,1)}, inner sep=0pt] (#1){};
    },
    gasmask/.pic = {
        \draw[rounded corners,line width=1pt] (0,0) arc (225:315:0.7) coordinate[pos=0.35] (s) coordinate[midway] (m) coordinate[pos=0.65] (e) coordinate[pos=1] (lr)
        -- +(0,0.6) coordinate[pos=0.60,xshift=-7pt] (r) arc (45:135:0.7) coordinate[pos=0] (ur) coordinate[pos=0.5] (um) coordinate[pos=1] (ul) -- (0,0) coordinate[pos=0.40,xshift=7pt] (l)-- cycle;
        \fill (m) circle (2mm);
        \draw[white] (m) circle (1.2mm);
        \fill (r) circle (1.4mm);
        \fill (l) circle (1.4mm);
        \fill[rotate=45] (s) rectangle +(-3mm,3mm);
        \fill[rotate=-45] (e) rectangle +(3mm,3mm);
        \node[fit={(0,0)([yshift=-1mm]m)(lr)(ur)(um)(ul)}, inner sep=0pt] (#1){};
    },
    meter/.pic = {
        \node[draw=black!50,fill=black!5,circle,inner sep=0pt,minimum width=8mm] (#1) at (0,0) {};
        \foreach \x [count=\c, evaluate=\x as \x using \x-40] in {0,17.3,...,260}{
            \pgfmathsetmacro{\xn}{mod(\c-1,5) == 0 ? 3.5 : 2.85};
            \pgfmathsetmacro{\cl}{\c < 7};
            \if\cl1 \edef\clr{red!70!black} \else \edef\clr{green!60!black} \fi
            \draw[\clr] ([shift=(\x:2mm)]#1.center) -- ([shift=(\x:\xn mm)]#1.center);
        }
        \draw[draw=black!50] ([shift=(220:2mm)]#1.center) arc (220:-40:2mm);
        \fill[rotate=-97] ([shift=(-105:2.75mm)]#1.center) -- ([shift=(-75:2.75mm)]#1.center) -- ([shift=(90:4mm)]#1.center);
        \draw[draw=black!50,thick,fill=black!5] (#1) circle (0.8mm);
        \node[font=\sffamily\tiny,anchor=south,yshift=-0.5mm] at (#1.south) {GAS};
    },
    pipe/.pic = {
        \draw[fill=black!50,draw=black] (0,0) -- (0.5,0) arc(225:315:0.5) -- ++(0.5,0) -- ++(0,0.5) coordinate[pos=0](#1-r) -- ++ (-0.5,0) arc(45:135:0.5) coordinate[pos=1] (#1-topl) coordinate[pos=0.5] (#1-top) coordinate[pos=0] (#1-topr) -- (0,0.5) -- cycle;
        \begin{scope}
            \clip (#1-topr) arc(45:135:0.5) (#1-topl) -- ++(0,1) -- ++(1,0) -- (#1-topr);
            \draw[draw=black,fill=black!50] ([xshift=-0.05cm,yshift=-0.1cm]#1-top) rectangle ([xshift=+0.05cm,yshift=0.4cm]#1-top);
        \end{scope}
        \draw[draw=black,fill=black!50,rounded corners=0.5pt] ([yshift=0.35cm]#1-topl) rectangle ([yshift=0.5cm]#1-topr);
        \node[fit={(0,-0.15cm)([yshift=1.1cm]#1-r)}, inner sep=0pt] (#1){};
    },
    pics/ccache/.style args = {#1/#2/#3/#4/#5/#6}{
        code = {
            \begin{scope}[shift=(#1),rotate=#4,yscale=#2]
                \pgfmathsetmacro\steps{#5+1}
                \pgfmathsetmacro\step{#3/\steps}
                \pgfmathsetmacro\filled{\step*(\steps-#6)}
                \foreach \m in {1,...,\steps}{
                    \draw[black!30] (\step * \m:0.475cm) -- +(\step * \m:0.25cm);
                }
                \draw (0:0.45cm) arc (0:#3:0.45cm) -- +({#3:0.30cm}) arc (#3:0:0.75cm) -- cycle;
                \fill[black!75] (#3:0.525cm) arc (#3:\filled:0.525cm) -- +({\filled:0.15cm}) arc (\filled:#3:0.70cm) -- cycle;
            \end{scope}
        }
    },
    pics/topo/.style args = {#1/#2/#3/#4}{
        code = {
            \pgfdeclarelayer{background}
            \pgfdeclarelayer{foreground}
            \pgfsetlayers{background,main,foreground}

            \node[root] (#1-R) {\texttt{R} \nodepart{lower} $1$};
            \node[#2,shift={(25:\DIST)}] (#1-A) at (#1-R) {$\mathtt{A}$};
            \node[#3,shift={(-45:\DIST)}] (#1-B) at (#1-R) {$\mathtt{B}$};
            \node[node,shift={(-15:\DIST)}] (#1-C) at (#1-A) {$\mathtt{C}$};
            \node[node,shift={(0:\DIST)}] (#1-D) at (#1-B) {$\mathtt{D}$};
            \node[node,shift={(65:\DIST)}] (#1-E) at (#1-C) {$\mathtt{A}$};
            \pic {ccache=t-D/-1/60/30/8/#4};
            \node[anchor=south west,yshift=1mm] at (#1-D.north east) {Cache};

            \pic[black!75] at ([yshift=0mm,xshift=-8mm]#1-E.west) {meter=#1-meter};
            %\path[-,densely dotted] (t-E) edge (t-meter);

            \node[cl,shift={(90:5em)}] (#1-CL) at (#1-R) {Cloud};
            \pic[black!75] at ([shift={(-130:7em)}]#1-CL) {tablet=#1-DV};

            \begin{pgfonlayer}{background}
                \draw let \p1 = (#1-R), \p2 = ([yshift=1pt]#1-CL.north), \n1 = {\y2-\y1} in coordinate (upper edge) at ([xshift=\n1,yshift=1pt]#1-CL.north);
                \draw let \p1 = ([xshift=-2pt]#1-R -| #1-DV.west), \p2 = (#1-R), \n1 = {\x1-\x2} in coordinate (lower edge) at ([xshift=-2pt,yshift=\n1]#1-R -| #1-DV.west);
                \coordinate (start) at ($(#1-R.45) + (45:0.3em)$);
                \coordinate (middle edge) at (upper edge -| lower edge);
                \coordinate (end) at ($(#1-R.225) + (225:0.3em)$);
                \fill[mqttBG] (start) -- (upper edge) -- (middle edge) -- (lower edge) -- node[above,pos=0.54] {MQTT} node[below,pos=0.54] {NDN} (end);
                \draw[black!30] (start) -- (upper edge) (end) -- (lower edge);
            \end{pgfonlayer}
        }
    },
    router/.style = {circle,minimum width=4pt,draw=black,fill=blue!20,inner sep=0pt},
    gw/.style = {router,regular polygon, regular polygon sides=3,fill=red!30,minimum width=7pt},
    tablet/.pic = {
        \filldraw[rounded corners=2pt,fill=white] (0,0) rectangle (0.75,1);
        \filldraw[fill=white] (0.12,0.2) rectangle (0.65,0.88);
        \fill (0.375,0.1) circle (1pt);
        \fill (0.375,0.4) circle (1pt);
        \draw
            ([shift=(45:0.1)]0.375,0.4) arc (45:135:0.1)
            ([shift=(45:0.175)]0.375,0.4) arc (45:135:0.175)
            ([shift=(45:0.25)]0.375,0.4) arc (45:135:0.25);
        \node[fit={(0,0)(0.75,1)}, inner sep=0pt] (#1){};
    },
    alarm/.pic = {
        \node (#1-bottom) [draw=black!75,fill=gray,trapezium, trapezium angle=87,minimum width=10,minimum height=2,trapezium stretches=true,draw,inner sep=1pt] {};
        \draw [draw=black!75,fill=red!100] (#1-bottom.163) [rounded corners=1pt] -- ++(0,0.28cm) -- ([yshift=0.28cm]#1-bottom.17) [sharp corners] -- (#1-bottom.17);
        \fill[black!40!red] ([xshift=-0.035cm,yshift=0.15cm]#1-bottom.north) ellipse (0.025 and 0.05);
        \fill[black!40!red] ([xshift=+0.035cm,yshift=0.15cm]#1-bottom.north) ellipse (0.025 and 0.05);
        \draw[black!40!red,line cap=round] ([yshift=0.015cm]#1-bottom.north) -- ++(0,0.2);
        \node[fit={(#1-bottom)([yshift=0.28cm]#1-bottom.north)}, inner sep=0pt] (#1){};
    },
    temp/.pic = {
        \draw[draw=black!75,fill=red!100] (0,0) arc (120:420:0.3) coordinate[pos=0.5] (#1-bottom) -- ++(0,0.60) coordinate (#1-tempr) -- (0,0.60) coordinate (#1-templ) -- (0,0);
        \draw[draw=black!75,fill=white] (#1-tempr) -- ++(0,0.4) coordinate (#1-topr) -- ([yshift=0.4cm]#1-templ) coordinate (#1-topl) -- (#1-templ);
        \node[fit={(#1-bottom)(#1-topl)(#1-topr)}, inner sep=0pt] (#1){};
    },
    pics/desktop/.style args = {#1/#2/#3}{
        code = {
            \draw[rounded corners=2pt,draw=black!100,fill=black!15] (0,0.2) rectangle (0.75,0.7);
            \draw[rounded corners=2pt,draw=black!100,fill=black!2] (0.05,0.3) rectangle (0.7,0.65);
            \node[font=\sffamily\tiny,inner sep=0pt, scale=#3, transform shape,align=center] at (0.375,0.47) {#2};
            \draw[draw=black!100,fill=black!15] (0.20,0) -- (0.55,0) -- ++(0,0.05) to[bend left] (0.4,0.2) -- ++(-0.05,0) to[bend left] (0.20,0.05) -- cycle;
            \fill (0.375,0.25) circle(0.5pt);
            \node[fit={(0,0)(0.75,0.7)}, inner sep=0pt] (#1){};
        }
    },
    db/.style={cylinder,cylinder uses custom fill,cylinder body fill=yellow!25, cylinder end fill=yellow!15,shape border rotate=90,aspect=0.25,draw=black!100,font=\sffamily\tiny,minimum width=0.35cm},
    network/.style = {cloud,cloud puffs=15.7,cloud ignores aspect,fill=black!15,draw=black!75,minimum width=1.75cm,minimum height=0.9cm, inner sep=0pt},
    scenario/.pic = {
        \draw (2.25,0) -- ++(0,1.25) arc (0:180:0.5) coordinate[pos=0.8] (#1-a) -- ++(0,-1.25) -- cycle;
        \draw [fill=white] (0,0) [rounded corners] -- (0,1) [sharp corners] --
              +(0.3,0.3) -- ++(0.3,0) --
              +(0.3,0.3) -- ++(0.3,0) --
              +(0.3,0.3) -- ++(0.3,0) --
              ++(0.1,0) coordinate (#1-b) [rounded corners] -- (2,1) [sharp corners] --
              (2,0) [sharp corners] -- cycle;
        \draw [fill=white] (2.1,0) [rounded corners] -- ++(0,1) --
              coordinate[pos=0.5] (#1-c) ++(1,0) [sharp corners] -- ++(0,-1) -- cycle;
        \draw (#1-c) -- ++(85:0.4) -- ++(0.175,0) coordinate (#1-d) -- ++(-85:0.4);
        \node[cloud, cloud puffs=12.7,cloud ignores aspect,fill=black!35, opacity=0.2, minimum width=0.3cm,minimum height=0.2cm, inner sep=0pt] at ([yshift=0.1cm]#1-d) {};
        \node[cloud, cloud puffs=13.7,cloud ignores aspect,fill=black!35, opacity=0.1, minimum width=0.4cm,minimum height=0.2cm, inner sep=0pt] at ([xshift=0.075cm,yshift=0.15cm]#1-d) {};
        \begin{scope}
            \clip (2.25,0) -- ++(0,1.25) arc (0:180:0.5) -- ++(0,-1.25) --
            (current bounding box.south west) -- (current bounding box.north west) --
            (current bounding box.north east) -- (current bounding box.south east) -- cycle;
            \draw[very thick,rounded corners] ([xshift=1]#1-a) -| (#1-b);
        \end{scope}
        \node[router] (#1-r2) at (35:1.0) {};
        \node[router] (#1-r4) at (25:1.5) {};
        \node[router] (#1-r5) at (18:2.5) {};
        \pic[scale=0.35,transform shape] at (73:0.70) {meter=#1-m1};
        \pic[scale=0.225] at (4:2.65) {pipe=#1-p1};
        \pic[scale=0.70,transform shape] at (30:0.275) {alarm=#1-a1};
        \pic[scale=0.16] at (4:2.3) {temp=#1-temp1};
        \node[gw] (#1-gw) at (40:2.25) {};
        \node [anchor=west,inner sep=1pt,font=\sffamily\tiny,scale=0.75,transform shape] at (#1-gw.45) {GW};
        \path[draw=black]
            (#1-r2) edge[draw=gray,decorate,decoration={expanding waves,angle=40,segment length=3.3}] ($(#1-a1.45)!0.5!(#1-m1.0)$)
            (#1-r2) edge (#1-r4)
            (#1-r5) edge[draw=gray,decorate,decoration={expanding waves,angle=40,segment length=3.2}] ($(#1-p1.90)!0.5!(#1-temp1.90)$)
            (#1-r4) edge (#1-gw)
            (#1-r5) edge (#1-gw)
        ;
        \node[network] (#1-network) at ([xshift=-0.35cm,yshift=1cm]#1-gw) {};
        \node[font=\sffamily\tiny,anchor=south east,inner sep=1pt,scale=0.75,transform shape,text=black!75] at (2,0) {Industrial Plant};
    },
}

